Mathematical Program Networks

Mathematical Program Networks (MPNs) are introduced in this work. An MPN is a collection of interdependent Mathematical Programs (MPs) which are to be solved simultaneously, while respecting the connectivity pattern of the network defining their relationships. The network structure of an MPN impacts which decision variables each constituent mathematical program can influence, either directly or indirectly via solution graph constraints representing optimal decisions for their decedents. Many existing problem formulations can be formulated as MPNs, including Nash Equilibrium problems, multilevel optimization problems, and Equilibrium Programs with Equilibrium Constraints (EPECs), among others. The equilibrium points of an MPN correspond with the equilibrium points or solutions of these other problems. By thinking of a collection of decision problems as an MPN, a common definition of equilibrium can be used regardless of relationship between problems, and the same algorithms can be used to compute solutions. The presented framework facilitates modeling flexibility and analysis of various equilibrium points in problems involving multiple mathematical programs.

==> deprecated/old.tex <==




% Note that $F_S(x)$ contains the origin only if $x\in S$. The contingent cone at $x\in\closed{S}$ is defined as 
% \begin{equation}
%     T_S(x) := \{ d \in\R{n} : \exists d_k \to d \text{ and } t_k \downarrow 0 \text{ with } x + t_k d_k \in S \}.
% \end{equation}
% For a convex set $C$, it is known that
% \begin{equation}
%     T_C(x) = \closed{F_C(x)} = F_{\closed{C}}(x).
% \end{equation}



% \begin{lemma}\label{lemma:convex_opt}
% If $S\subset \R{n}$ is a convex set, and $p\in\R{n}$, then $\ip{p}{d} \ge 0  \ \forall d \in F_S(x)$ if and only if $\ip{p}{d} \ge 0  \ \forall d \in F_{\closed{S}}(x)$.
% % then $x^*$ is a locally optimal solution to (\ref{eq:basic_opt}) if and only if $\ip{\nabla f(x^*)}{d} \ge 0, \ \forall d\in F_{\closed{S}}(x^*)$.
% \end{lemma}
% \begin{proof}
% Since $F_S(x^*) \subset F_{\closed{S}}(x^*)$, the \emph{if} direction is clear. To demonstrate the \emph{only if} direction, consider some $d\in F_{\closed{S}}(x^*)$, such that $\ip{p}{d} < 0$. Let $\hat{d} \in F_S(x)$. Define $d_\epsilon := (1-\epsilon)d + \epsilon \hat{d}$. It follows that $d_\epsilon \in F_S(x^*) \ \forall \epsilon > 0$ by the convexity of $S$. But $\ip{p}{d_\epsilon} < 0$ for small enough $\epsilon$, implying that if $\exists d \in F_{\closed{S}}(x)$ with $\ip{p}{d} < 0$, then there exists $\exists d_\epsilon \in F_{S}(x)$ with $\ip{p}{d_\epsilon} < 0$, proving the claim.
% \end{proof}
% The normal cone of $C$ at $x$ is defined as the polar set of the tangent cone:
% \begin{equation}
%     N_C(x) := (T_C(x))^\circ.
% \end{equation}

% The following property will be used in later results:

% \begin{lemma} \label{lemma:1}
% For any convex set $C \subset \R{n}$,
% $(\bar{C})^\circ = C^\circ$.
% \end{lemma}
% \begin{proof}
% Because $C\subset \bar{C}$, it follows immediately that $(\bar{C})^\circ \subset C^\circ$. To show the other direction, suppose there exists some $v\in C^\circ, \ v\notin (\bar{C})^\circ$. In other words, $v \in C^\circ$ but $\exists e \in (\bar{C} \setminus C)$ with $\ip{v}{e} > 0$. Let $d \in C$. Then $\ip{v}{d} \leq 0$. Cince $(\bar{C} \setminus C)$ is closed, the vector $e_\epsilon := (1-\epsilon)e + \epsilon d \in C, \forall \epsilon > 0$. But for small enough $\epsilon$, $\ip{v}{e_\epsilon} > 0$. This implies $v\notin C^\circ$, a contradiction. Therefore $v\in C^\circ \implies v \in (\bar{C})^\circ$. 
% \end{proof}



% \begin{proof}
% Because $\interior{S} \subset S$, it follows immediately that $S^\circ \subset (\interior{S})^\circ$. To show the other direction, suppose there exists some $v\in (\interior{S})^\circ, \ v\notin S^\circ$. In other words, $v\in (\interior{S})^\circ$ but $\exists e \in \partial S$ with $\ip{v}{e} > 0$. Let $d \in \interior{S}$. Then $\ip{v}{d} \leq 0$. Since $\partial S$ is closed, the vector $e_\epsilon := (1-\epsilon)e + \epsilon d \in \interior{S}, \forall \epsilon > 0$. But for small enough $\epsilon$, $\ip{v}{e_\epsilon} >0$. This implies $v\notin (\interior{S})^\circ$, a contradiction. Therefore $v\in (\interior{S})^\circ \implies  v \in S^\circ$.
% \end{proof}

% \begin{lemma} \label{lemma:convex_opt}
% If $C\subset \R{n}$ is a closed convex set, and $f$ is a convex function, $x^*\in C$ is an optimal solution to the problem $\min_{x\in C} f(x)$ if and only if \begin{equation}
%     -\nabla_x f(x^*) \in N_C(x^*).
% \end{equation}
% \end{lemma}

% The following corollary is a direct consequence of \cref{lemma:1,lemma:convex_opt}.
% \begin{corollary} \label{cor:feas}
% If $C\subset \R{n}$ is a convex set (not-necessarily closed), and $f$ is a convex function, $x^*\in \bar{C}$ is an optimal solution to the problem $\min_{x\in \bar{C}} f(x)$ if and only if \begin{equation}
%     -\nabla_x f(x^*) \in (F_C(x^*))^\circ.
% \end{equation}
% \end{corollary}

% For a given positive integer $N$, consider the following collection of parametric optimization problems, defined for $i\in\{1,\hdots,N\}$:

% \begin{equation}
% \begin{aligned}
%     \min_{x^i} \ \ &f_i(x) \\
%     \text{s.t.} \ \ &x \in S_i.
% \end{aligned}
% \end{equation}

% Here, $x^i \in \R{n_i}$, and the problem is parameterized by $x^{-i}$, the decision variables for all other problems $j\ne i$ in the collection. Specifically, let $n=\sum_{i=1}^N n_i$, and
% \begin{equation}
%     x^{-i} := (x^1,...,x^{i-1},x^{i+1},...,x^N) \in \R{n-n_i}.
% \end{equation}

% \begin{definition}[Generalized Nash Equilibrium]

% \end{definition}



\subsection{Single-player opt: union of convex regions}

Consider a mathematical program of the following form:

\begin{equation}
    \label{mp:simple}
    \begin{aligned}
        &\min_{x\in\R{n}} \mathrlap{ \ \ \ f(x) }\\
        &\ \ \text{s.t.} & x &\in S,
    \end{aligned}
    % \tag{$\mathrm{MP}$}
\end{equation}

where $f$ is a convex function, and 

\begin{equation}
    S := \bigcup_{j\in \mathcal{J}} S_j.
\end{equation}

% \begin{equation} \label{eq:open_poly}
%     S_j := \big\{ x \in\R{n} : \langle s_{j,k}, x \rangle + t_{j,k} \bowtie_k 0, \ k \in \{1,...,p_j\} \big\}.
% \end{equation}

% Here, $p_j > 0$ represents the number of half-spaces comprising $S_j$, $s_{j,k}\in\R{n}$, $t_{j,k}\in\R{}$, and $\bowtie_k \in \{ \geq, > \}$. Hence, each affine inequality may or may not be strict. 

Here $\mathcal{J}$ is some index set of finite cardinality, and each $S_j$ is a non-empty, convex, not-necessarily closed, polyhedron. For each $j\in\mathcal{J}$, a related mathematical program can be defined:

\begin{equation}
    \label{mp:simplej}
    \begin{aligned}
        &\min_{x\in\R{n}} \mathrlap{ \ \ \ f(x) }\\
        &\ \ \text{s.t.} & x &\in \bar{S}_j.
    \end{aligned}
    % \tag{$\mathrm{MP}_j$}
\end{equation}

Define $I_{\bar{S}} : \R{n} \to \mathcal{P}(\mathcal{J})$ as
\begin{equation}
    I_{\bar{S}}(x) := \{ j \in \mathcal{J} : x \in \bar{S}_j \}.
\end{equation} 

The following result relates solutions of problem (\ref{mp:simple}) to those of problems (\ref{mp:simplej}). 

\begin{theorem} \label{thm:1}
$x^*$ is a local optimum of (\ref{mp:simple}) if and only if $x^* \in S$ and $x^*$ is an optimum of (\ref{mp:simplej}) for all $j \in I_{\closed{S}}(x^*)$.
\end{theorem}

\begin{proof}
First note that \begin{equation}
    F_S(x^*) \le := \bigcup_{j\in\J} F_{S_j}(x^*) = \bigcup_{j\in I_{\closed{S}}(x^*)} F_{S_j}(x^*),
\end{equation} since $F_{S_j}(x^*) = \emptyset \ \forall j \notin I_{\closed{S}}(x^*)$. Hence by \cref{lemma:simple_opt}, if $x^*$ is a local optimum for \cref{mp:simple}, then $\ip{\nabla f(x^*)}{d} \ge 0, \ \forall d \in F_{S_j}(x^*), \ \forall j \in I_{\closed{S}}(x^*)$. But by \cref{lemma:convex_opt}, this condition is equivalent to $\ip{\nabla f(x^*)}{d} \ge 0, \ \forall d \in F_{\closed{S}_j}(x^*), \ \forall j \in I_{\closed{S}}(x^*)$. Because $x^* \in \closed{S}_j$ for all such $j$, this is again equivalent by \cref{lemma:simple_opt} to $x^*$ being a local optimum of (\ref{mp:simplej}) for all $j \in I_{\closed{S}}(x^*)$.

Suppose now that $x^*$ is not a local optimum of (\ref{mp:simple}). Then $\exists x\in S \cap B_\epsilon(x^*)$ with $f(x^*) > f(x)$. Let $k \notin I_{\closed{S}}(x^*)$. Then $x^* \notin \closed{S}_k$. Because $\closed{S}_k$ is a closed set, $(\closed{S}_k)'$ is open, and hence $x^* + d \notin \closed{S}_k$ for all $\|d\| < \epsilon$. Since this is true for any $k\notin I_{\closed{S}}(x^*)$, this implies $I_{\closed{S}}(x^*+d) = I_{\closed{S}}(x^*)$ for all $\|d\| < \epsilon$. Therefore $S \cap B_\epsilon(x^*) = (\cup_{i\in I_{\closed{S}}(x^*)} S_i) \cap B_\epsilon(x^*)$. Therefore there must be some $j\in I_{\closed{S}}(x^*)$ such that $f(x^*) > f(x)$ with $x \in S_j$. Therefore if $x^*$ is not a local optimum of (\ref{mp:simple}), then $x^*$ cannot be a local optimum of (\ref{mp:simplej}) for all $j \in I_{\closed{S}}(x^*)$. 
%  First assume that $x^*\in S$ is an optimum of \cref{mp:simplej} for all $j \in \IS(x^*)$, implying $f(x^*) \leq f(y), \ \forall y \in \closed{S}_j$. Now for every  $i \notin \IS(x^*)$, we have $x^* \notin \closed{S}_i \implies x^* \in (\closed{S}_i)'$ (the complement of $\closed{S}_i$). Because $(\closed{S}_i)'$ is an open set, there exists some $\epsilon > 0$ such that $x^* + d \in (\closed{S}_i)'$, or equivalently $x^*+d \notin \closed{S}_i$ for all $\|d\| < \epsilon$. This implies that $\IS(x^*+d) \subset \IS(x^*)$ for all such $d$. It follows that  
% \begin{equation} \label{eq:subsets_implies}
% (\Be(x^*) \cap S) \subset (\Be(x^*) \cap \bar{S}) \subset \left(\Be(x^*) \cap \cup_{j\in\IS(x^*)} \bar{S}_j\right) \subset \cup_{j\in\IS(x^*)} \bar{S}_j
% \end{equation}
% Here, $\Be(x^*)$ is an open $\epsilon$-ball containing $x^*$. Now by the initial assumption, $f(x^*) \leq f(y), \ \forall y \in \cup_{j\in\IS(x^*)} \bar{S}_j$, which by \cref{eq:subsets_implies} implies $f(x^*) \leq f(y), \ \forall y \in (\Be(x^*) \cap S)$, which is the definition of a local optimum for \cref{mp:simple}. 

% ($\impliedby$) Now suppose $x^*$ is a local optimum of \cref{mp:simple} (therefore it must be that $x^* \in S$), but $\exists j \in \IS(x^*)$ and $y\in \bar{S}_j$ such that $f(y) < f(x^*)$ (so that $x^*$ is not a local optimum for \cref{mp:simplej}). By \cref{cor:feas}, it must be that $-\nabla_x f(x^*) \notin (F_{S_j}(x^*))^\circ$. But this implies that there exists $d \in F_{S_j}(x^*),$ such that $\ip{-\nabla_x f(x^*)}{d} > 0$, or $\ip{\nabla_x f(x^*)}{d} < 0$. This implies that for small enough $\epsilon > 0$, $x^* + \epsilon d \in S$ and $f(x^*+\epsilon d) < f(x^*)$, contradicting the assumption that $x^*$ is a local optimum of \cref{mp:simple}.
\end{proof}

\subsection{Multi-player equilibria}

Consider a collection of $N$ parametric optimization problems, one for each $i$ in the index set $\N := \{1,\hdots,N\}$.

\begin{equation}
    \label{eq:simple}
    \begin{aligned}
        \min_{x^i} \ &f_i(x) \\
        \text{s.t.} \ &x \in C_i \\
        &x \in S
    \end{aligned}
\end{equation}


\begin{equation}
    \label[mp]{mp:eq}
    \begin{aligned}
        % SOL_i(w, x^{-i}, y^{-i}) := \
        &\ \ \min_{x^i, y^i} \mathrlap{ \ \ \ f_i(
        w,x,y^i) }\\
        &\ \ \ \ \text{s.t.} && (w,x,y^i) \in C_i \\
        &&&  (w,x,y^i) \in S \\
        &&& y^i = y^1,  &(i \ne 1) \\
        &&& y^i = y^{j\ne1}, &(i = 1) \\
    \end{aligned} \tag{$\mathrm{PMP}_i$}
\end{equation}

Here, $x^i \in \R{n_i}$ is the private decision variable associated with $\PMP_i$, and $y^i\in\R{p}$ is a private copy of a \emph{negotiated} decision variable shared among the $N$ programs. Let $n = \sum_{i\in\N} n_i$. Each of the $N$ problems are parameterized by $w \in \R{m}$, as well as $x^{-i}$ and $y^{-i}$, where
\begin{equation}
    x^{-i} := (x^1,...,x^{i-1},x^{i+1},...,x^N) \in \R{n-n_i},
\end{equation}
and $y^{-i}$ is defined analogously.
  The pair $(x^i, x^{-i})$ should be taken to be $x:=(x^1,...,x^N)\in\R{n}$. The function $f_i : \R{m+n+p} \to \R{}$ is a convex quadratic function. Note that unlike the sets $C_i$, the set $S$ is the same in each of the $N$ problems, and is defined as in the previous section:
\begin{equation}
    S := \bigcup_{j\in \J} S_j.
\end{equation}
$\J$ is an index set of finite cardinality. The sets $S_j, A_i \subset \R{m+n+p}$ are non-empty, not-necessarily closed, convex polyhedra. 
% For each \cref{mp:eq}, the set-valued correspondence $SOL_i : \R{m+n+Np} \to \mathcal{P}(\R{n_i+p})$ defines the set of local optima.
% \begin{equation}
% \begin{aligned}
%     SOL_i(w,\hat{x},\hat{y}) := \{ &(x^i,y^i) : \\
%     &f_i\left(w,(x^i,\hat{x}^{-i}),(y^i,\hat{y}^{-i})\right) \leq f_i\left(w,(\tilde{x}^i,\hat{x}^{-i}),(\tilde{y}^i,\hat{y}^{-i})\right),
%     &\forall 
% \end{aligned}
% \end{equation}



As before, related parametric mathematical programs can be defined for each $j\in\J$:

 \begin{equation}
    \label[mp]{mp:eqj}
    \begin{aligned}
        % SOL_{i,j}(w,x^{-i}, y^{-i}) := \
        &\ \ \min_{x^i, y^i} \mathrlap{ \ \ \ f_i(
        w,x,y^i) }\\
        &\ \ \ \ \text{s.t.} && (w,x,y^i) \in \bar{C}_i \\
        &&&  (w,x,y^i) \in \bar{S}_j \\
        &&& y^i = y^1,  &(i \ne 1) \\
        &&& y^i = y^{j\ne1},  &(i = 1) \\
    \end{aligned} \tag{$\mathrm{PMP}_{i,j}$}
\end{equation}

\begin{definition}[Generalized Nash Equilibrium] 
For a given $w\in\R{m}$, $(x^*,y^*)$ is a generalized Nash equilibrium point for problems $\{\mathrm{PMP}_i\}_{i\in\N}$, if and only if $((x^*)^i, (y^*)^i) \in SOL_i(w,x^*,y^*)$.
\end{definition}

% Specifically, let 
% \begin{equation}
%     A_i := \big\{ (w,x,y) : \langle a_{i,k}, (w,x,y) \rangle + b_{i,k} \bowtie_k 0, \ k \in \{1,...,K_{A_i}\} \big\}
% \end{equation}
% \begin{equation}
%     S_j := \big\{ (w,x,y) : \langle s_{j,k}, (w,x,y) \rangle + t_{j,k} \bowtie_k 0, \ k \in \{1,...,K_{S_j}\} \big\},
% \end{equation}

% where $a_{i,k},s_{j,k} \in \R{m+n+p}$ and $\bowtie_k \in \{ \geq, > \}$. These sets need not be in minimal representation. 

% Let the closure of some set $M$ be denoted $\bar{M}$. Now for each each $j\in J$, a similar collection of problems can be defined:

%

% Let the function $I : \R{m+n+p} \to \mathcal{P}(J)$ (where $\mathcal{P}(J)$ denotes the power set of $J$) be given by
% \begin{equation}
%     I_{\bar{S}}(w,x,y) := \{j\in J : (w,x,y) \in \bar{S}_j\}.
% \end{equation}

% The first important result can now be stated.

% \begin{lemma}
% $((x^i)^*,y^*) \in \mathrm{MP}_i(x^{-i}, w)$ if and only if $(w,(x^i)^*,x^{-i},y^*) \in S$ and $((x^i)^*,y^*) \in \mathrm{MP}_{i,j}(x^{-i}, w)$ for all $j \in I_{\bar{S}}(w,(x^i)^*,x^{-i},y^*)$.
% \end{lemma}


==> deprecated/prelim.tex <==
The following notation is used throughout the remainder of this paper. Consider a set $S \subset \R{n}$. The closure of $S$ is denoted $\bar{S}$, the complement of $S$ ($\R{n} \setminus S$) is denoted $S'$, the interior of $S$ ($\R{n} \setminus \closed{(\R{n} \setminus S)}$) is $\interior{S}$, and the boundary of $S$ ($\closed{S} \setminus \interior{S}$) is denoted $\partial S$. The polar set of $S$ ($\{v\in\R{n} : \langle v,d\rangle \leq 0 \ \forall d \in S\}$) is denoted $S^\circ$. For any set $G$ (infinite or finite), the power set of $G$ is denoted $\mathcal{P}(G)$.

For a set $S \subset \R{n}$, the set of feasible directions at some point $x\in\closed{S}$ is defined as 
\begin{equation}
    F_S(x) := \{ d\in\R{n} : \exists t_k \downarrow 0, \text{ with } x+t_k d \in S\}.
    % \exists d_k \to d \text{ and } t_k \downarrow 0 \text{ with } x + t_k d_k \in C \}.
\end{equation}

Note that for a convex set $C$, $F_{\closed{C}}(x) = \closed{F_C(x)}$. 
% Note that $F_S(x)$ contains the origin only if $x\in S$. The contingent cone at $x\in\closed{S}$ is defined as 
% \begin{equation}
%     T_S(x) := \{ d \in\R{n} : \exists d_k \to d \text{ and } t_k \downarrow 0 \text{ with } x + t_k d_k \in S \}.
% \end{equation}
% For a convex set $C$, it is known that
% \begin{equation}
%     T_C(x) = \closed{F_C(x)} = F_{\closed{C}}(x).
% \end{equation}

\begin{lemma}\label{lemma:simple_opt}
Consider the optimization problem, 
\begin{equation} \label{eq:basic_opt}
    \min_{x \in S} f(x),
\end{equation}
where $f$ is continuously differentiable and $S\subset \R{n}$. If $x^* \in S$ is a locally optimal solution, then $\ip{\nabla f(x^*)}{d} \ge 0, \ \forall d\in F_S(x^*)$. If $f$ and the set $S$ are both convex, then $x^* \in S$ is a locally optimal solution if and only if $\ip{\nabla f(x^*)}{d} \ge 0, \ \forall d\in F_S(x^*)$
\end{lemma}

\begin{lemma}\label{lemma:convex_opt}
If $S\subset \R{n}$ is a convex set, and $p\in\R{n}$, then $\ip{p}{d} \ge 0  \ \forall d \in F_S(x)$ if and only if $\ip{p}{d} \ge 0  \ \forall d \in F_{\closed{S}}(x)$.
% then $x^*$ is a locally optimal solution to (\ref{eq:basic_opt}) if and only if $\ip{\nabla f(x^*)}{d} \ge 0, \ \forall d\in F_{\closed{S}}(x^*)$.
\end{lemma}
\begin{proof}
Since $F_S(x^*) \subset F_{\closed{S}}(x^*)$, the \emph{if} direction is clear. To demonstrate the \emph{only if} direction, consider some $d\in F_{\closed{S}}(x^*)$, such that $\ip{p}{d} < 0$. Let $\hat{d} \in F_S(x)$. Define $d_\epsilon := (1-\epsilon)d + \epsilon \hat{d}$. It follows that $d_\epsilon \in F_S(x^*) \ \forall \epsilon > 0$ by the convexity of $S$. But $\ip{p}{d_\epsilon} < 0$ for small enough $\epsilon$, implying that if $\exists d \in F_{\closed{S}}(x)$ with $\ip{p}{d} < 0$, then there exists $\exists d_\epsilon \in F_{S}(x)$ with $\ip{p}{d_\epsilon} < 0$, proving the claim.
\end{proof}
% The normal cone of $C$ at $x$ is defined as the polar set of the tangent cone:
% \begin{equation}
%     N_C(x) := (T_C(x))^\circ.
% \end{equation}

% The following property will be used in later results:

% \begin{lemma} \label{lemma:1}
% For any convex set $C \subset \R{n}$,
% $(\bar{C})^\circ = C^\circ$.
% \end{lemma}
% \begin{proof}
% Because $C\subset \bar{C}$, it follows immediately that $(\bar{C})^\circ \subset C^\circ$. To show the other direction, suppose there exists some $v\in C^\circ, \ v\notin (\bar{C})^\circ$. In other words, $v \in C^\circ$ but $\exists e \in (\bar{C} \setminus C)$ with $\ip{v}{e} > 0$. Let $d \in C$. Then $\ip{v}{d} \leq 0$. Cince $(\bar{C} \setminus C)$ is closed, the vector $e_\epsilon := (1-\epsilon)e + \epsilon d \in C, \forall \epsilon > 0$. But for small enough $\epsilon$, $\ip{v}{e_\epsilon} > 0$. This implies $v\notin C^\circ$, a contradiction. Therefore $v\in C^\circ \implies v \in (\bar{C})^\circ$. 
% \end{proof}



% \begin{proof}
% Because $\interior{S} \subset S$, it follows immediately that $S^\circ \subset (\interior{S})^\circ$. To show the other direction, suppose there exists some $v\in (\interior{S})^\circ, \ v\notin S^\circ$. In other words, $v\in (\interior{S})^\circ$ but $\exists e \in \partial S$ with $\ip{v}{e} > 0$. Let $d \in \interior{S}$. Then $\ip{v}{d} \leq 0$. Since $\partial S$ is closed, the vector $e_\epsilon := (1-\epsilon)e + \epsilon d \in \interior{S}, \forall \epsilon > 0$. But for small enough $\epsilon$, $\ip{v}{e_\epsilon} >0$. This implies $v\notin (\interior{S})^\circ$, a contradiction. Therefore $v\in (\interior{S})^\circ \implies  v \in S^\circ$.
% \end{proof}

% \begin{lemma} \label{lemma:convex_opt}
% If $C\subset \R{n}$ is a closed convex set, and $f$ is a convex function, $x^*\in C$ is an optimal solution to the problem $\min_{x\in C} f(x)$ if and only if \begin{equation}
%     -\nabla_x f(x^*) \in N_C(x^*).
% \end{equation}
% \end{lemma}

% The following corollary is a direct consequence of \cref{lemma:1,lemma:convex_opt}.
% \begin{corollary} \label{cor:feas}
% If $C\subset \R{n}$ is a convex set (not-necessarily closed), and $f$ is a convex function, $x^*\in \bar{C}$ is an optimal solution to the problem $\min_{x\in \bar{C}} f(x)$ if and only if \begin{equation}
%     -\nabla_x f(x^*) \in (F_C(x^*))^\circ.
% \end{equation}
% \end{corollary}

% For a given positive integer $N$, consider the following collection of parametric optimization problems, defined for $i\in\{1,\hdots,N\}$:

% \begin{equation}
% \begin{aligned}
%     \min_{x^i} \ \ &f_i(x) \\
%     \text{s.t.} \ \ &x \in S_i.
% \end{aligned}
% \end{equation}

% Here, $x^i \in \R{n_i}$, and the problem is parameterized by $x^{-i}$, the decision variables for all other problems $j\ne i$ in the collection. Specifically, let $n=\sum_{i=1}^N n_i$, and
% \begin{equation}
%     x^{-i} := (x^1,...,x^{i-1},x^{i+1},...,x^N) \in \R{n-n_i}.
% \end{equation}

% \begin{definition}[Generalized Nash Equilibrium]

% \end{definition}


==> intro.tex <==
\begin{figure}[t]
    \centering
    \fbox{\includegraphics[angle=-90,origin=c,width=0.90\linewidth]{figures/front_fig.png}}
    \caption{A four-node Mathematical Program Network. Each node attempts to minimize a cost function $f^i$ while satisfying the constraints represented by $C^i$ as well as those which are imposed by the network structure. An equilibrium is any point which is an element of all four solution graphs $S^i$, which in this case is equivalent to being an element of $S^1$.}
    \label{fig:front}
\end{figure}



The optimization problem is ubiquitous as a modeling construct because of its simultaneous simplicity and expressivity. Especially for well-studied classes of problems, such as Linear Programs or Convex Quadratic Programs, practitioners find utility in the knowing that any problem stated as one of these instances (of moderate dimension and conditioning) will be efficiently solvable to global optimality. Staying within the modeling restrictions specified by the problem class, one can modify the objective or constraint functions of the program to better produce desired output, and can rest assured that those changes will not impact the fundamental solvability or solution properties of their program. 

There are of course more generalized optimization problems which do not have the same properties. Generally, only local optimality is tenable for non-convex optimization problems, and even this may not be true for non-smooth problems or those with integer variables. These formulations offer more modeling flexibility, but at the cost of less reliable or efficient solution properties. 

Not all generalizations of, say, Convex Quadratic Programs can even be modeled as proper optimization problems---convex, continuous or otherwise. For example, Bimatrix games can be seen to be generalizations of Quadratic Programs, in which two QPs are defined in relation to each other, and must be solved simultaneously to an equilibrium point. These instances listed can be reduced to a more general formulation, the Linear Complementarity Problem, which under certain assumptions also offers efficient computation of solutions, which may also be unique or connected as in its QP counterpart. Nevertheless, these relatively simple problems do not fit into the constrained framework of optimization. 

Similarly, one can generalize QPs by combining multiple instances in a different manner, namely as in Bilevel optimization. When the top and bottom programs of a Bilevel program are both (when considered independently) convex QPs, again the structure inherent in the problem can be exploited to find solutions efficiently. Comparing Bilevel problems and two-player Generalized Nash games, both are combinations of two related QPs, differing only by the nature of the relationship between them. These two problems are exemplars of two primary mechanisms for relating QPs, namely \emph{flat} and \emph{nested} relationships. 

Some other lesser-common but still well-known formulations containing multiple constituent QPs exhibit these same relationships. Consider, for example, the Feedback Nash equilibrium of an inequality-constrained LQ game. This problem can be seen to be a series of Nash equilibrium problems (flat connections), successively played over time (nested connections). Other instances which combine both patterns in the QP setting include Quadratic Programs with Linear Complementarity constraints, or Nash Equilibrium Problems with Nash Equilibrium Constraints (multi-leader-multi-follower games). In these less-common formulations, solution approaches are not well developed, and those approaches that do exist often exploit specific assumptions about the connectivity pattern of the problem.


% 2. Game theoretic formulations: notions of equilibrium generalize optimality, and study the interaction of multiple decision makers. Obvious examples are Nash eq and Bilevel optimization (Stackelberg eq). Less common examples are Feedback Nash eq, etc. Practitioners of game theoretic methods will be familiar with the restriction that decision structure places on modeling freedom. E.g. might want to change a flat formulation to a nested formulation, but not possible in current modeling frameworks and solvers. 

With this in mind, it is natural to consider a generalized framework for modeling and solving networks of connected QPs. In such a framework, the relationship between decision problems becomes first-class aspect of modeling---changes to the relationship between constituent QPs would not fundamentally change the ability for solution approaches to compute solutions. The utility of such a formulation, and importantly, of reliable and efficient solution algorithms, would be invaluable. Many readers will intuit correctly that in the worst-case, it will be computationally intractable to compute solutions for general networks of QPs. However, as it will be demonstrated in this article, many applications of interest do not suffer this problem, and the existence of hard examples should not deter from the study or development of algorithms devoted to their solution. 

In this paper, the concept of a Quadratic Program Network is introduced, which is as aleueded to, a collection of Quadratic Programs, each of which are related to each other by either flat or nested connections. The contributions made by this work are the following. First, the QP Net framework is introduced, highlighting many interesting and real-world problems which can naturally be modeled as QPNets. Equilibrium points for QPNets are defined, and various properties about QPNets are proved. Importantly, an algorithm is also introduced and evaluated on a small suite of example problems. Open source software is released which is capable of conveniently modeling QPNets in the Julia language, and can compute equilibrium points efficiently. 

==> motivation.tex <==
% To motivate the development of MPNs, a simple example is used to illustrate that the same group of mathematical programs generally have different equilibrium points when considered under different network architectures, and therefore each node in an MPN will have a preference on how the network is arranged. To explore the importance that network architecture has on resulting cost of equilibrium, a small-scale class of randomly generated \emph{Constellation Games} are presented. 

\subsection{Constellation Game Case Study} \label{sec:motivation}

A simple example is presented here to illustrate that the same group of mathematical programs generally have different equilibrium points when considered under different network architectures, and therefore each node in an MPN will have a preference on how the network is arranged. To explore the importance that network architecture has on resulting cost of equilibrium, a small-scale class of randomly generated \emph{Constellation Games} are presented. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/four_player_example/constellations.png}
    \caption{A depiction of each node's cost function for a randomly generated constellation game. Each constellation (depicted by a color) indicates how a particular node would decide $\mathbf{x}$ if it had unconstrained control over the entire vector. The differently oriented triangles are used to indicate different sub-vectors of $\mathbf{x}$.
    }
    \label{fig:constellations}
\end{figure}

\begin{example}[Constellation Game] \label{example:constellation_game}
    Consider a MPN described by the following table:
    \renewcommand{\arraystretch}{1.6}
    \begin{center}
    \begin{tabular}{ |c c|  }
     \hline
     Dec. vars: & $\mathbf{x} := \left[ \p^1, \p^2, \p^3, \p^4 \right], \ \p^i \in \R{2}$ \\[2pt]
     \hline \hline
     \multicolumn{2}{|c|}{ Nodes $i \in \{1,2,3,4\}$: } \\\hline
     Cost: & $\|{\mathbf{x}}^i - \mathbf{g}^{i}\|_2^2 + \sum_{j=1,j\ne i}^4 \| {\mathbf{x}}^j - {\mathbf{x}}^i - \mathbf{r}^{i,j}\|_2^2$ \\
     Feasible set: & $\{ \mathbf{x}: \|\p^i\|_\infty \le 5 \}$ \\
     Private vars: & $\p^i$ \\
     Child nodes: & ? \\
     \hline
    \end{tabular}
    \end{center}
\end{example}



The particular example used here is comprised of four MP nodes, indexed $1$ through $4$. The decision index sets for these MPs are given by 
\begin{equation*}
   J^1 := \{1,2\}, \ \ J^2 := \{3,4\}, \ \ J^3 := \{5,6\}, \ \ J^4 := \{7,8\},
\end{equation*}
and as such the total decision space dimension is given by $n=8$. The feasible set for each of the nodes is a box over their respective decision spaces, lifted into $\mathbb{R}^8$:
\begin{equation*}
    C^i := \{ \mathbf{x} \in \mathbb{R}^8 : -5 \le x_j \le 5, \ \ \forall j \in J^i \}.
\end{equation*}

The cost function for each node is of the following form:
\begin{equation*}
    f^i(\mathbf{x}) := \|{\mathbf{x}}^i - \mathbf{g}^{i}\|_2^2 + \sum_{j=1,j\ne i}^4 \| {\mathbf{x}}^j - {\mathbf{x}}^i - \mathbf{r}^{i,j}\|_2^2,
\end{equation*}
where the vectors $\mathbf{g}^i$ are target locations, and the vectors $\mathbf{r}^{i,j}$ are target relationships between the vectors ${\mathbf{x}}^i$ and ${\mathbf{x}}^j$.  

In the analysis below, each instance of this class of constellation game is generated by sampling the vectors $\mathbf{g}^i$, $\mathbf{r}^{i,j}$ from the standard unit multivariate normal distribution:
\begin{equation*}
   \mathbf{g}^{i} \sim \mathcal{N}(\mathbf{0}, \mathbf{I}), \ \  \mathbf{r}^{i,j} \sim \mathcal{N}(\mathbf{0}, \mathbf{I}).
\end{equation*}
A depiction of the cost function for each of the four nodes can be seen in \cref{fig:constellations} for a particular random sampling of the target and relationship vectors. 

Using the four nodes so far described, different MPNs can be constructed by relating the nodes with various network architectures. Each of these MPNs correspond to selecting a set of network edges from the super-set of all possible directed edges (excluding self edges):
 \begin{equation*}
    E^{\mathrm{super}} := \left\{ (i,j) : i \in [4], j \in [4], i \ne j \right\}
    % \begin{aligned}
    % &(1,2), (1,3), (1,4), (2,1), (2,3), (2,4),\\
    % &(3,1), (3,2), (3,4), (4,1), (4,2), (4,3)
    % \end{aligned} \right\}.
\end{equation*}

 There are 12 elements in $E^\mathrm{super}$, and therefore $2^{12}=4096$ ways to construct a network architecture for a four-node MPN in this manner. However, for this analysis, only acyclic networks are considered, since cyclic networks result in degenerate MPNs as discussed in \cref{sec:formulation}. Furthermore, some sets of edges can contain redundant edges, meaning the set of reachable transitions $\mathbf{R}$ for a network is unchanged if those edges are removed. Edge sets with redundant edges are also not considered in this analysis. 

Due to symmetry of the nodes in this game, many of the remaining MPNs can also be removed from consideration. From the perspective of any particular node, the other three nodes are interchangeable under a permutation of decision indices. For example, from the perspective of node $1$, the networks defined by edge sets $\{(1,2),(2,3)\}$ and $\{(1,4),(4,2)\}$ are identical (until the goal and relationship vectors are realized). Only network architectures in which node $1$ is uniquely oriented with respect to its interchangable peers are included. 

After removing the cyclic and redundant configurations as defined, there are only $47$ remaining configurations to be analyzed. These network configurations are shown in \cref{fig:four_node_example}, with the yellow-colored node indicating the location of node $1$. As stated, the impact that various network architectures have on the  yellow node can be used to understand the impact on all other nodes in the constellation game as well via a symmetry argument.

Having these 47 unique network configurations identified, a randomized analysis of the benefit that each architecture provides for a given node was performed. To accomplish this, multiple instances of the constellation game were randomly sampled. For each instance, and for each of the 47 network configurations, an equilibrium was computed (using the methods described in TODO section), and the cost incurred for node 1 at this equilibrium point was logged. Aggregating over 50,000 random game instances, the average cost reduction compared to the Nash equilibrium (the empty edge set) for each of the other configurations was computed, along with the standard error, from which $95\%$ confidence intervals on the average cost estimate could be generated. These cost estimates are displayed for each of the network configurations in \cref{fig:four_node_example}. 

The resulting ordering of network architectures, from most to least advantageous for a given node, is rather fascinating. The Nash configuration with no edges is the worst (all other configurations provide an advantage in comparison). The best configuration, with $6.24\%$ reduction in average cost relative to the Nash configuration is the four-level network with node $1$ as the single source node. Interestingly, a four-level network with node $1$ appearing further down the hierarchy is still significantly better than many other configurations in which node $1$ is a source node, sometimes even the only source node. For example, the edge configuration $\{(2,3),(3,4),(4,1)\}$ (7th best) has a $5.19\%$ cost reduction, while the configuration $\{(1,2),(1,3),(1,4)\}$ (11th best) has a $4.64\%$ reduction. 

One conclusion that could be made from these results is that a hierarchical network configuration is advantageous for all nodes in an MPN, even for the nodes at the bottom of the hierarchy. Seemingly it is better to be at the bottom of a strongly hierarchical configuration than it is to be at the top of a configuration in which a clear hierarchy is not established. This is at least true for the constellation game example explored here. Understanding the role that network configuration has on all MPNs is a topic that should be explored in later work. 

\SetTblrInner{rowsep=2.9pt}
\SetTblrInner{colsep=3pt}

\begin{figure}  \centering
\begin{tblr}{|c|c|c|c|c|}
    \hline 
\csname graph22\endcsname &
\csname graph21\endcsname &
\csname graph23\endcsname &
\csname graph43\endcsname &
\csname graph29\endcsname \\
(-6.24±0.08)\% &
(-5.87±0.07)\% &
(-5.72±0.10)\% &
(-5.48±0.06)\% &
(-5.40±0.11)\% \\\hline
\csname graph19\endcsname &
\csname graph40\endcsname &
\csname graph18\endcsname &
\csname graph37\endcsname &
\csname graph45\endcsname \\
(-5.37±0.10)\% &
(-5.19±0.11)\% &
(-5.07±0.05)\% &
(-4.83±0.11)\% &
(-4.72±0.10)\% \\\hline
\csname graph17\endcsname &
\csname graph46\endcsname &
\csname graph26\endcsname &
\csname graph34\endcsname &
\csname graph35\endcsname \\
(-4.64±0.04)\% &
(-4.45±0.10)\% &
(-4.34±0.09)\% &
(-4.10±0.09)\% &
(-4.08±0.09)\% \\\hline
\csname graph33\endcsname &
\csname graph24\endcsname &
\csname graph27\endcsname &
\csname graph44\endcsname &
\csname graph41\endcsname \\
(-3.70±0.09)\% &
(-3.69±0.07)\% &
(-3.34±0.08)\% &
(-3.31±0.06)\% &
(-3.12±0.08)\% \\\hline
\csname graph25\endcsname &
\csname graph47\endcsname &
\csname graph28\endcsname &
\csname graph32\endcsname &
\csname graph20\endcsname \\
(-2.85±0.05)\% &
(-2.73±0.07)\% &
(-2.53±0.06)\% &
(-2.52±0.06)\% &
(-2.43±0.04)\% \\\hline
\csname graph6\endcsname &
\csname graph39\endcsname &
\csname graph7\endcsname &
\csname graph30\endcsname &
\csname graph5\endcsname \\
(-2.40±0.04)\% &
(-2.29±0.07)\% &
(-2.07±0.05)\% &
(-2.07±0.05)\% &
(-1.95±0.03)\% \\\hline
\csname graph38\endcsname &
\csname graph36\endcsname &
\csname graph12\endcsname &
\csname graph13\endcsname &
\csname graph31\endcsname \\
(-1.88±0.06)\% &
(-1.86±0.06)\% &
(-1.86±0.06)\% &
(-1.84±0.06)\% &
(-1.63±0.05)\% \\\hline
\csname graph42\endcsname &
\csname graph10\endcsname &
\csname graph11\endcsname &
\csname graph9\endcsname &
\csname graph8\endcsname \\
(-1.42±0.05)\% &
(-1.42±0.05)\% &
(-1.41±0.05)\% &
(-1.19±0.03)\% &
(-1.17±0.03)\% \\\hline
\csname graph16\endcsname &
\csname graph15\endcsname &
\csname graph14\endcsname &
\csname graph2\endcsname &
\csname graph3\endcsname \\
(-0.98±0.04)\% &
(-0.98±0.04)\% &
(-0.98±0.04)\% &
(-0.70±0.02)\% &
(-0.49±0.03)\% \\\hline
\csname graph4\endcsname &
\csname graph1\endcsname & & & \\
(-0.48±0.03)\% & 0\% & & & \\\hline
\end{tblr}
\caption{The 47 unique network configurations for the constellation game described in \cref{sec:motivation}, arranged in order of best to worst for the yellow-colored node. Equilibrium points were found for each configuration, for each of 50,000 random instances of the game. The average relative cost reduction (for the yellow node) compared to the Nash equilibrium (the edgeless configuration) and associated 95\% confidence interval are given for each network configuration.}
\label{fig:four_node_example}
\end{figure}
